Efficient and Scalable Graph Pattern Mining on GPUs

Graph Pattern Mining (GPM) extracts higher-order information in a large graph by searching for small patterns of interest. GPM applications are computationally expensive, and thus attractive for GPU acceleration. Unfortunately, due to the complexity of GPM algorithms and parallel hardware, hand optimizing GPM applications suffers programming complexity, while existing GPM frameworks sacrifice efficiency for programmability. Moreover, little work has been done on GPU to scale GPM computation to large problem sizes. We describe G2Miner, the first Graph Pattern Mining (GPM) framework that runs on multiple GPUs. G2Miner uses pattern-aware, input-aware and architecture-aware search strategies to achieve high efficiency on GPUs. To simplify programming, it provides a code generator that automatically generates pattern-aware CUDA code. G2Miner flexibly supports both breadth-first search (BFS) and depth-first search (DFS) to maximize memory utilization and generate sufficient parallelism for GPUs. For the scalability of G2Miner, we use a customized scheduling policy to balance work among multiple GPUs. Experiments on a V100 GPU show that G2Miner achieves average speedups of 5.4x and 7.2x over two state-of-the-art single-GPU systems, Pangolin and PBE, respectively. In the multi-GPU setting, G2Miner achieves linear speedups from 1 to 8 GPUs, for various patterns and data graphs. We also show that G2Miner on a V100 GPU is 48.3x and 15.2x faster than the state-of-the-art CPU-based system, Peregrine and GraphZero, on a 56-core CPU machine.

==> tbl-optimizations-old.tex <==
\begin{table}[]
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{r|ccc|c|c|c}
\Xhline{2\arrayrulewidth}
 & \multicolumn{3}{c|}{\textbf{Enabled in \sys by}} & \multirow{2}{*}{\textbf{Pangolin}} & \multirow{2}{*}{\textbf{PBE}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}{\bf Third-party} \\ \textbf{applications}\end{tabular}} \\ \cline{2-4}
 & \multicolumn{1}{c}{input} & \multicolumn{1}{c}{pattern} & \multicolumn{1}{c|}{arch} & & & \\ 
\Xhline{2\arrayrulewidth}
\multicolumn{1}{l|}{P: Data graph preprocessing~\cref{sect:interface}} & & \checkmark & & \checkmark & NA & \cite{DistTC,KClique} \\ \hline
%\multicolumn{1}{l|}{Data graph ordering~\cref{sect:interface}} & & & & NA & NA & \cite{Peregrine,GraphZero} \\
\multicolumn{1}{l|}{\hlp{C}: Two-level parallelism~\cref{sect:parallelism}} & & & \checkmark & NA & NA & \cite{DistTC} TC only\\
\multicolumn{1}{l|}{\hlp{C}: Hybrid order on GPU~\cref{sect:orders}} &  & \checkmark & \checkmark & NA & NA & NA \\
\multicolumn{1}{l|}{\hlp{C}: Multi-pattern fission~\cref{sect:optimization}(1)} & & \checkmark & \checkmark & NA & NA & NA \\
\multicolumn{1}{l|}{\hlp{C}: Counting-only pruning~\cref{sect:optimization}(2)} & & \checkmark & & NA & NA & \cite{DwarvesGraph} CPU only\\
\multicolumn{1}{l|}{\hlp{C}: Local graph search~\cref{sect:optimization}(3)} & \checkmark & \checkmark & & NA & NA & \cite{KClique} CL only\\ \hline
\multicolumn{1}{l|}{\hlb{L}: SIMD-aware primitives~\cref{sect:primitives}(1)} & & & \checkmark & NA & NA & NA \\
\multicolumn{1}{l|}{\hlb{L}: Flexible data format~\cref{sect:primitives}(2)} & \checkmark & \checkmark & & NA & NA & \cite{kclique-gpu} CC only \\ \hline
\multicolumn{1}{l|}{\hlr{R}: Multi-gpu scheduling~\cref{sect:scheduler}} & & \checkmark & & NA & NA & \cite{Rossi} MC only \\
\multicolumn{1}{l|}{\hlr{R}: Data graph partition~\cref{sect:mem-mgmt}(1)} & \checkmark & \checkmark & & NA & \checkmark & \cite{DUALSIM} CPU only \\
\multicolumn{1}{l|}{\hlr{R}: Edgelist reduction~\cref{sect:mem-mgmt}(2)} & & \checkmark & & NA & NA & NA \\
\multicolumn{1}{l|}{\hlr{R}: Adaptive buffering~\cref{sect:mem-mgmt}(3)} & \checkmark & \checkmark & \checkmark & NA & NA & NA \\ 
\multicolumn{1}{l|}{\hlr{R}: Mem. save for FSM~\cref{sect:mem-mgmt}(4)} & \checkmark & \checkmark & & NA & NA & NA \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{Optimizations enabled in \sys. They are done in the preprocessor ({P}), code generator (\hlp{C}), primitive library (\hlb{L}) and runtime system (\hlr{R}).
NA: not available. TC: triangle counting. CL/CC: clique listing/counting. MC: motif counting.}
\label{tab:optimizations}
\end{table}

==> tbl-optimizations-speedup.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl|ccccc|c|c|c|c}
\hline
\multicolumn{2}{c|}{}                                                                                                                                                                                                                                   & \multicolumn{5}{c|}{\textbf{Effect}}                                                                                                                                                                                                                                                                                                                                                                    &                                    &                                                                                             &                                                                                                  &                                                                                                  \\ \cline{3-7}
\multicolumn{2}{c|}{\multirow{-2}{*}{\textbf{Optimizations}}}                                                                                                                                                                                           & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}mitigate\\ divergence\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}load\\ balancing\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}memory\\ saving\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}algorithmic\\ pruning\end{tabular}} & \begin{tabular}[c]{@{}c@{}}extra GPU\\ efficiency\end{tabular} & \multirow{-2}{*}{\textbf{Speedup}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Available\\ in Pangolin?\end{tabular}}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Used in hand \\ written apps?\end{tabular}}} & \multirow{-2}{*}{\textbf{Conditions to apply}}                                                   \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Category-(1):\\ Known\end{tabular}}}                                                                  & \begin{tabular}[c]{@{}l@{}}A: Data graph preprocessing\\ (edge orientation)\end{tabular} & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{\checkmark}                                                     &   & 2.6x                               & \checkmark                                                                                   & \checkmark                                                                                        & cliques                                                                                          \\ \hline
\multicolumn{1}{c|}{}                                                                                                                                        & B: Data graph partitioning                                                               & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{\textbf{}}                                                     &  &                                    & x                                                                                           & TC only                                                                                          & \begin{tabular}[c]{@{}c@{}}hub patterns, graph size, \\ GPU memory size\end{tabular}             \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & C: Two-level parallelism                                                                 & \multicolumn{1}{c|}{\checkmark}                                                     & \multicolumn{1}{c|}{\checkmark}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{\textbf{}}                                                     & \textbf{}                                                      & 5.4x                               & x                                                                                           & TC only                                                                                          & always enabled on GPU                                                                            \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & D: Counting-only pruning                                                                 & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{\checkmark}                                                     & \textbf{}                                                      & 6.2x                               & x                                                                                           & CPU only                                                                                         & \begin{tabular}[c]{@{}c@{}}automatic pattern \\ decomposition {[}83{]}\end{tabular}              \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & E: Local graph search                                                                    & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{\checkmark}                                                     & \textbf{}                                                      &                                    & x                                                                                           & CL only                                                                                          &                                                                                                  \\ \cline{2-7} \cline{9-10}
\multicolumn{1}{c|}{}                                                                                                                                        & F: Flexible data format                                                                  & \multicolumn{1}{c|}{\checkmark}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      & \multirow{-2}{*}{2.1x}             & x                                                                                           & CC only                                                                                          & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}hub patterns \&\\ ∆ \textless 1024\end{tabular}}     \\ \cline{2-11} 
\multicolumn{1}{c|}{\multirow{-6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Category-(2):\\ \\ Known, but not \\ enabled in prior \\ GPM systems\end{tabular}}}} & G: Multi-gpu scheduling                                                                  & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\checkmark}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      & Fig.9                              & x                                                                                           & MC only                                                                                          & always used on multi-GPU                                                                         \\ \hline
\multicolumn{1}{c|}{}                                                                                                                                        & {\color[HTML]{000000} H: SIMD-aware primitives}                                          & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{}                                                              & \checkmark                                                      & 1.7x                               & x                                                                                           & x                                                                                                & \begin{tabular}[c]{@{}c@{}}hardware support for \\ warp level primitives\end{tabular}            \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & {\color[HTML]{000000} I: Multi-pattern fission}                                          & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\textbf{}}                                               & \multicolumn{1}{c|}{}                                                              & \checkmark                                                      & 1.2x                               & x                                                                                           & x                                                                                                & \begin{tabular}[c]{@{}c@{}}explicit multi-pattern \& \\ kernel occupancy by NVCC\end{tabular}    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & {\color[HTML]{000000} J: Edgelist reduction}                                             & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      &                                    & x                                                                                           & x                                                                                                & if v0 \textgreater v1 in symmetry order                                                          \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & {\color[HTML]{000000} K: Adaptive buffering}                                             & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      &                                    & x                                                                                           & x                                                                                                & \begin{tabular}[c]{@{}c@{}}buffer W usage in matching \\ order \& GPU memory size\end{tabular}   \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                                                                        & {\color[HTML]{000000} M: Hybrid order on GPU}                                            & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      &                                    & x                                                                                           & x                                                                                                & \begin{tabular}[c]{@{}c@{}}implicit, intermediate data \\ unbounded, user-specified\end{tabular} \\ \cline{2-11} 
\multicolumn{1}{c|}{\multirow{-6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Category-(3):\\ \\ Novel\end{tabular}}}}                                             & {\color[HTML]{000000} N: Mem. save for FSM}                                              & \multicolumn{1}{c|}{\textbf{}}                                                     & \multicolumn{1}{c|}{\textbf{}}                                                & \multicolumn{1}{c|}{\checkmark}                                               & \multicolumn{1}{c|}{}                                                              & \textbf{}                                                      &                                    & x                                                                                           & x                                                                                                & \begin{tabular}[c]{@{}c@{}}implicit, vertex label \\ frequency, user-specified\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Optimizations in G2Miner. Among them, optimizations A,B,D,E,F,I,J,K,M,N are pattern-aware; optimizations B,C,G,H,I,K,M are architecture-aware; optimizations B,E,F,K,N are input-aware.}
\label{tab:optimizations}
\end{table*}

==> user-code-tc.tex <==

\begin{lstlisting}[
float=tp,floatplacement=t,
xleftmargin=0.5in,
linewidth=7.9cm,
label={lst:tc},
basicstyle=\ttfamily\footnotesize,
language=C++, 
abovecaptionskip=0pt,
%frame = single, 
firstnumber = last, 
escapeinside={(*@}{@*)},
escapeinside={(*}{*)},
morekeywords = {Vertex, Graph, Subgraph, Pattern, Set, Map, Match, void, int, int64},
caption = {Triangle Counting (TC) user code in \sys}]
Graph G = loadDataGraph("graph.csr");
Pattern p = generateClique(3);
int64 result = count(G, p);
\end{lstlisting}

==> vldb-block.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> vldb-command.tex <==

%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{XX.XX/XXX.XX}
\newcommand\vldbpages{XXX-XXX}
% issue-specific
\newcommand\vldbvolume{14}
\newcommand\vldbissue{1}
\newcommand\vldbyear{2020}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{URL_TO_YOUR_ARTIFACTS}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{plain} 

==> workload-model.tex <==
\noindent
{\it Workload Estimation}.
It is difficult to know the workload for each task without actually running it, 
since the workload of a task depends on the graph topology as well as the pattern.
For example, for the pattern of \texttt{triangle}, the workload of a task, i.e., an edge ($v_1$, $v_2$), is the intersection of $v_1$ and $v_2$'s neighborhood, which is $O(d_{v_1}+d_{v_2})$. 
%where $M$ and $N$ are $v_1$'s degree and $v_2$'s degree respectively.
However, if given a larger pattern, the amount of work would involve neighborhoods within more hops, making it more difficult to estimate.

Consider the subgraph search tree in \cref{fig:subgraph-tree}. 
%We denote $N_{i+1}$ as 
The number of subgraphs at level $i+1$ that are extended from a subgraph ($v_1$, $v_2$, ..., $v_i$) at level $i$ is $\sum_{w=v_1}^{v_i} d(w)$.
Given a size $k$ pattern, the workload of a task $e$=($v_1$, $v_2$) is $(d_{v_1}+d_{v_2}) \times \prod_{hop=1}^{k-3} \sum_{w \in nghbr(hop,e)} d(w)$,
where $nghbr(j, e)$ represents the $j$ hop neighborhood of edge $e$.
Apparently this equation is too expensive to compute in practice.
Instead, we can approximate it to do the estimation: $d_{v_1}+d_{v_2}$.
This is cheap to compute, and our experiments in \cref{sect:eval} show that this estimation is accurate enough for our use.
For the vertex-parallel mode, we use $d_{v_1}$ to estimate workload of task $v_1$.
